Anti-Path Cover on Sparse Graph Classes

We show that it is possible to use Bondy-Chvatal closure to design an FPT algorithm that decides whether or not it is possible to cover vertices of an input graph by at most k vertex disjoint paths in the complement of the input graph. More precisely, we show that if a graph has tree-width at most w and its complement is closed under Bondy-Chvatal closure, then it is possible to bound neighborhood diversity of the complement by a function of w only. A simpler proof where tree-depth is used instead of tree-width is also presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{82}
\providecommand{\publicationstatus}{J. Bouda et al. (Eds.): 11th Doctoral Workshop\\
on  Mathematical and Engineering Methods\\
in Computer Science (MEMICS 2016)\\
EPTCS 233, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.233.8}{10.4204/EPTCS.233.8}}
\pdfoutput=1

